The DUNE Far Detector Interim Design Report, Volume 2: Single-Phase Module

The DUNE IDR describes the proposed physics program and technical designs of the DUNE far detector modules in preparation for the full TDR to be published in 2019. It is intended as an intermediate milestone on the path to a full TDR, justifying the technical choices that flow down from the high-level physics goals through requirements at all levels of the Project. These design choices will enable the DUNE experiment to make the ground-breaking discoveries that will help to answer fundamental physics questions. Volume 2 describes the single-phase module's subsystems, the technical coordination required for its design, construction, installation, and integration, and its organizational structure.

==> common/intro.tex <==
% Intro shared by all subsections NOT USED IN TECNICAL PROPOSAL

\section{An International Physics Program}

The global neutrino physics community is developing a multi-decade
physics program to measure unknown parameters of the Standard Model of
particle physics and search for new phenomena.  The program will be carried out as an international,
leading-edge, dual-site experiment for neutrino science and proton decay studies, which 
is known as the Deep Underground Neutrino Experiment (DUNE).
The detectors for this experiment will be designed, built, commissioned and operated by the international DUNE Collaboration. The facility required to support this experiment, the Long-Baseline Neutrino Facility (LBNF), is hosted by Fermilab and its design and construction is organized as a DOE/Fermilab project incorporating international partners. Together LBNF and DUNE will comprise the world's highest-intensity neutrino beam at Fermilab, in Batavia, IL, a high-precision near detector on the Fermilab site, a massive liquid argon time-projection chamber (LArTPC) far detector installed deep underground at the Sanford Underground Research Facility (SURF) \SI{1300}{\km} away in Lead, SD, and all of the conventional and technical facilities necessary to support the beamline and detector systems. 


The strategy for executing the experimental program presented in this Technical
Design Report (TDR) has been developed to meet the requirements 
set out in the P5 report~\cite{p5report} and takes into account the recommendations of the European Strategy for Particle Physics~\cite{ESPP-2012}. It adopts a model where U.S. and international funding agencies 
share costs on the DUNE detectors, and CERN and other participants provide in-kind contributions 
to the supporting infrastructure of LBNF. LBNF and DUNE have been and will remain tightly coordinated as DUNE collaborators 
develop the detectors and infrastructure that will carry out the scientific program.
  
The scope of LBNF is
\begin{itemize}
\item an intense neutrino beam aimed at the far site,
\item a beamline measurement system
\item conventional facilities at both the near and far sites, and
\item cryogenics infrastructure to support the DUNE detector at the far site.
\end{itemize}

The DUNE detectors include
\begin{itemize}
\item a high-performance neutrino detector 
located a few hundred meters downstream of the neutrino source, and
\item a massive liquid argon time-projection chamber (LArTPC) neutrino detector located deep underground at the far site.
\end{itemize}

With the facilities provided by LBNF and the detectors provided by
DUNE, the DUNE Collaboration proposes to mount a focused attack on the
puzzle of neutrinos with broad sensitivity to neutrino oscillation
parameters in a single experiment.  The focus of the scientific
program is the determination of the neutrino mass hierarchy and the
explicit demonstration of leptonic CP violation, if it exists, by
precisely measuring differences between the oscillations of muon-type
neutrinos and antineutrinos into electron-type neutrinos and
antineutrinos, respectively. Siting the far detector deep underground
will provide exciting additional research opportunities in nucleon
decay, studies utilizing atmospheric neutrinos, and neutrino
astrophysics, including measurements of neutrinos from a core-collapse
supernova should such an event occur in our galaxy during the
experiment's lifetime.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{The LBNF/DUNE Technical Design Report Volumes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A Roadmap of the TDR}

The LBNF/DUNE TDR describes the proposed physics program and \fixme{baselined?}
technical designs.

The TDR is composed of \fixme{some number of} volumes and is supplemented by several annexes that 
provide details on the physics program and technical designs. The volumes are as follows

\begin{itemize}
\item \volintro{}\cite{tdr-vol-1} provides an executive summary of and strategy for the experimental 
program and introduces the TDR.
\item \volphys{}\cite{tdr-vol-2} outlines the scientific objectives and describes the physics studies that 
the DUNE Collaboration will undertake to address them.
\item \vollbnf{}\cite{tdr-vol-3} describes the LBNF Project, which includes design and construction of the 
beamline at Fermilab, the conventional facilities at both Fermilab and SURF, and the cryostat
 and cryogenics infrastructure required for the DUNE far detector.
\item \voldunenear{}\cite{tdr-vol-4}  describes design, construction and 
commissioning of the DUNE near detector. 
\item \voldunefar{}\cite{tdr-vol-5}  describes design, construction and 
commissioning of the DUNE far detectors.
\end{itemize}

More detailed information for each of these volumes is provided in a set of annexes listed on LBNF and DUNE's shared  \href{https://web.fnal.gov/project/LBNF/SitePages/Proposals%20and%20Design%20Reports.aspx}{\textit{Proposals and Design Reports} page}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{About this Volume}  <----- follows in overview chapter file of indiv volume



==> far-detector-generic/chapter-fd-coordination/outline-dp.tex <==
\chapter{Technical Coordination}
\label{ch:fdsp-coord}

\input{far-detector-generic/chapter-fd-coordination/intro}
\input{far-detector-generic/chapter-fd-coordination/support}
\input{far-detector-generic/chapter-fd-coordination/integration}
\input{far-detector-generic/chapter-fd-coordination/infrastructure}
\input{far-detector-generic/chapter-fd-coordination/itf}
\input{far-detector-generic/chapter-fd-coordination/installation}



==> far-detector-generic/chapter-generic-slow-and-cryo/cryo-instrum-cfd.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Cryogenics Instrumentation}
\label{sec:fdsp-cryo-instr} % label used for \ref's from single phase sections.
\label{sec:fddp-cryo-instr} % label used for \ref's from dual phase sections.
\label{sec:fdgen-cryo-instr} % label used for \ref's from generic sections.
% Jim G %Carmen

Instrumentation inside the cryostat must ensure that the condition of the \dword{lar} is adequate for operation of the \dshort{tpc}.
This instrumentation includes devices to monitor the impurity level of the argon, e.g., the purity monitors, which provide high precision electron lifetime measurements,
and gas analyzers to ensure that the levels of atmospheric contamination drop below certain limits during the cryostat purging, cooling and filling.
The cryogenics system operation is monitored by temperature sensors deployed in vertical arrays and at the top and bottom of the detector, providing a 
detailed \threed temperature map which can help to predict the \dword{lar} purity across the entire cryostat. The cryogenics instrumentation also includes \lar level monitors and
a system of internal cameras to help in locating sparks in the cryostat and for overall monitoring of the cryostat interior. 
As mentioned in the Introduction, cryogenics instrumentation requires simulation work to identify the proper location for these devices inside the cryostat and
for the coherent analysis of the instrumentation data. 

Figure~\ref{fig:sp-slow-cryo-ports} shows the current map of cryostat ports for the \dword{spmod}, highlighting the ones assigned to instrumentation devices,
as well as the preliminary location for some of these devices. Vertical temperature profilers are located behind the \dwords{apa} ($T_S$) and behind the east end wall ($T_D$).
They are complemented by a coarser \twod grid of sensors at the top and bottom of the cryostat (not shown in the figure). Purity monitors as well as level meters are planned
in each detector side, behind the two front end walls. Inspection cameras will use some of the multipurpose instrumentation ports, but their exact locations are yet to be decided. 

For \dual, additional care must be taken to monitor the gas phase above the liquid level as the temperature and pressure of argon gas affect gas pressure, and consequently the \dword{lem} calibration.  The gas pressure must be monitored to \SI{1}{mbar} precision and accuracy. In proximity to the liquid surface the temperature gradient of the  gas has to be measured with an array of temperature probes with a vertical pitch of about \SI{1}{cm}, and with a coarser \SI{5}{cm} pitch up to the cryostat roof. Each \dword{crp} is also equipped with \num{36} thermometers to sample the temperature across its structure.


\begin{dunefigure}[Cryostat ports]{fig:sp-slow-cryo-ports}
{Cryostat ports and preliminary location of some instrumentation devices. }
\includegraphics[width=0.95\textwidth]{cisc_cryostat_ports.png}
\end{dunefigure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Fluid Dynamics Simulations}
\label{sec:fdgen-slow-cryo-cfd}
% P. Strons
% S. Gollapinni

Proper placement of purity monitors, thermometers, and liquid level monitors within the \dword{detmodule} requires knowledge of how \dword{lar} behaves within the cryostat in terms of its fluid dynamics, heat and mass transfer, and distribution of impurity concentrations. 
Fluid motion within the cryostat is driven primarily by small changes in density from thermal gradients, although pump flow rates and inlet and outlet locations also contribute. 
Heat sources include exterior heat from the surroundings, interior heat from the electronics, and heat flow through the pump inlet.

The fluid flow behavior can be determined through simulation of \dword{lar} flow within the detector using ANSYS CFX\footnote{ANSYS\texttrademark{}, \url{https://www.ansys.com/products/fluids/ansys-cfx}.}, a commercially available \dfirst{cfd} code. Such a model must include proper definition of the fluid characteristics, solid bodies and fluid-solid interfaces, and a means for measuring contamination, while still maintaining reasonable solve times.
\fixme{compute times?}
Although simulation of the \dword{detmodule} presents challenges, there exist acceptable simplifications for accurately representing the fluid, the interfacing solid bodies, and variations of contaminant concentrations. Because of the magnitude of thermal variation within the cryostat, modeling of the \dword{lar} is simplified through use of constant thermophysical properties, calculation of buoyant force through use of the Boussinesq Model (using constant a density for the fluid with application of a temperature dependent buoyant force), and a standard shear stress transport turbulence model. Solid bodies that contact the \dword{lar} include the cryostat wall, the cathode planes, the anode planes, the ground plane, and the \dword{fc}. As in previous \dshort{cfd} models of the DUNE \dword{35t} and \dword{protodune} by South Dakota State University (SDSU)\cite{docdb-5915}, the \dword{fc} planes, anode planes, and \dword{gp} can be represented by porous bodies. Since impurity concentration and electron lifetime do not impact the fluid flow, these variables can be simulated as  passive scalars, as is commonly done for smoke releases~\cite{cfd-1} in air or dyes released in liquids.

\fixme{some of this sounds very SP to me -anne}

Significant discrepancies between real data and simulations can have potential impacts on detector performance, as simulation results contribute to decisions about where to locate sensors and monitors, as well as definitions of various calibration quantities. However, methods of mitigating such risks include well established convergence criteria, sensitivity studies, and comparison to results of previous \dshort{cfd} simulation work by SDSU and \fnal. Additionally, the simulation will be improved with input from temperature measurements and validation tests. 

%%%%% Must find better pictures. Just use this for now %%% anne to here Fri 4/27
\begin{dunefigure}[\dshort{cfd} example]{fig:cfd-example}
  {Distribution of temperature on a plane intersecting an inlet (right) and halfway between an inlet and an outlet (left), as predicted by SDSU \dshort{cfd} simulations \cite{docdb-5915}. (See Figure\ \ref{fig:cfd-example-geometry} for geometry.)}
  \includegraphics[height=0.4\textwidth]{cisc_cfd_outlet_z0.png}
  \includegraphics[height=0.4\textwidth]{cisc_cfd_inlet_z52.png}
\end{dunefigure}

Figure~\ref{fig:cfd-example} shows an example of the temperature
distribution on a plane intersecting a \dword{lar} inlet and at a
plane halfway between an inlet and an outlet; the geometry used for
this simulation is shown in Figure~\ref{fig:cfd-example-geometry}.
Note the plume of higher temperature \dword{lar} between the walls and
the outer \dword{apa} on the inlet plane.  The current locations of instrumentation in
the cryostat as shown in Figure~\ref{fig:sp-slow-cryo-ports} were
determined using the temperature and impurity distributions from these
previous simulations.

\begin{dunefigure}[\dshort{cfd} example geometry]{fig:cfd-example-geometry}
  {Layout of the \dshort{tpc} within the cryostat (top) and positions of
    \dword{lar} inlets and outlets (bottom) as modeled in the SDSU
    \dshort{cfd} simulations \cite{docdb-5915}.
    The Y axis is vertical and the X axis is parallel to the \dword{tpc}
    drift direction.
    Inlets are shown in green and outlets are shown in red.}
  \includegraphics[width=0.8\textwidth]{cisc_cfd_cryostat-layout}
  \includegraphics[width=0.8\textwidth]{cisc_cfd_inlet-outlet-layout}
\end{dunefigure}

The initial strategy for the future \dword{cfd} simulation effort is to understand the performance of \dword{protodune} cryogenics system and model the \dwords{fd} to derive requirements for instrumentation devices.
The following is a prioritized set of studies planned to help drive the requirements for other systems:
\begin{enumerate}
\item Review the DUNE \dword{fd} cryogenics system design and verify the current implementation in simulation; this is important to ensure that the model represents what will be built.
\item Model the \dword{pddp}  liquid and gas regions with the same precision as the \dword{fd}. Presently only the liquid model exists. The liquid model is needed to interpret the thermometer data, and the gas model is needed to understand how to place thermometers in the ullage and verify the design of the gaseous argon purge system.
\item Perform a \dword{cfd} study to determine the feasibility of a wier for \dual; this helps to determine if it can be used to clean the \lar surface before the extraction grid is submerged in the \dword{dpmod}.
\item Verify the \dword{spmod} \single \dword{cfd} model in simulation performed by LBNF; this defines the requirements for instrumentation devices (e.g., thermometry).
\item Model the \dword{pddp} liquid and gas regions with the same precision as the \dword{fd}. \fixme{same as a previous bullet}
\end{enumerate}


==> far-detector-single-phase/chapter-fdsp-performance.tex <==
\chapter{Detector Performance}
\label{ch:fdsp-perform}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{??}
\label{sec:fdsp-perform-??}

\section{Far Detector Optimization Studies}
\label{sec:fdsp-perform-optimization}

The DUNE Far Detector Task Force was formed in 2015 and charged with developing a complete simulation and reconstruction infrastructure, and using these tools in optimization studies of key detector parameters such as wire pitch and angle.  The final report of that task force was presented in 2017 and includes a number of results that help motivate the design of the DUNE-SP modules presented in this document.  Highlights from these optimization studies are presented in this section, and include comparisons of the following DUNE geometry arrangements:

\begin{itemize}
\item{\textbf{Default}: APAs with 5 mm wire pitch, and Induction wires at 36$^{\circ}$ angle.}
\item{\textbf{3mm}: APAs with 3 mm wire pitch, and Induction wires at 36$^{\circ}$ angle.}
\item{\textbf{45Deg}: APAs with 5 mm wire pitch, and Induction wires at 45$^{\circ}$ angle.}
\item{\textbf{r90DegBeam}: APAs with 5 mm wire pitch, and Induction wires at 36$^{\circ}$ angle, but with APAs effectively rotated 90 degrees from the beam axis.}  
\end{itemize}



\subsection{Tracking Efficiency}
\label{sec:fdsp-perform-trackingeff}



\begin{dunefigure}[Impact of APA geometry on muon/pion/proton tracking efficiency]{fig:fdsp-perform_trackingeff_optimization}{Tracking efficiency for $\mu^-$ (top-left), $\pi^+$ (top-right), $\pi^-$ (bottom-left), and $p$ (bottom-right) from charged-current interactions, shown for 4 arrangements of APA geometry.}
\includegraphics[width=0.85\textwidth]{TrackingEfficiency_GeometryOptimization.pdf}
\end{dunefigure}

\begin{dunefigure}[Tracking efficiency comparison between different reconstruction algorithms]{fig:fdsp-perform_trackingeff_comparison}{Tracking efficiency $K^+$ (top), $\mu^+$ (middle), and Michel electrons (bottom) using LineCluster (left) or TrajCluster (right), as a function of true particle length in proton decay events.}
\includegraphics[width=0.85\textwidth]{TrackingEfficiency_GeometryOptimization_TwoAlgorithms.pdf}
\end{dunefigure}

\subsection{Electron and Photon Reconstruction}
\label{sec:fdsp-perform-showerreco}

\begin{dunefigure}[Impact of APA geometry on electron/photon dE/dx reconstruction]{fig:fdsp-perform_dEdx_optimization}{Average dE/dx for electrons and photons, shown for 3 arrangements of DUNE APA  geometry.}
\includegraphics[width=0.6\textwidth]{dEdx.pdf}
\end{dunefigure}

\begin{dunefigure}[Impact of APA geometry on electron efficiency and photon rejection.]{fig:fdsp-perform_dEdx_optimization}{Impact of APA geometry on electron efficiency and photon rejection using a dE/dx vs. range selection approach.  Three APA configurations are shown.  The right plot is a zoomed-in view of the left plot.}
%\includegraphics[width=0.85\textwidth]{egamma_signalbackground_optimization.pdf}  reduce file size on image by DeMuth
\includegraphics[width=0.85\textwidth]{egamma_signalbackground_optimization.png}
\end{dunefigure}


\section{Lessons Learned for Single-Phase LArTPCs}
\label{sec:fdsp-perform-lessons}

DUNE-SP benefits from the collective experience of several previous LArTPC detectors, and many important lessons learned from those efforts have helped shape the design of the experiment.  Among these lessons are:

\begin{itemize}
\item{Improved knowledge of achieving and maintaining high-purity LAr.}
\item{Improved understanding of the impact of LAr purity on HV system performance.}
\item{Mitigation of high-voltage discharge damage through cathode design and surge-protection elements on the field-cage.}
\item{Offline software filtering to improve electronics signal/noise levels.}
\item{Anode design to protect against broken/shorted wires.}
\end{itemize}

\subsection{Impact of Operating Drift-Field}
\label{sec:fdsp-perform-drift}

The very long drift lengths inherent in the DUNE-SP design require that the combination of drift electric field and LAr purity are sufficient to minimize charge attenuation throughout the TPC.  The nominal operating electric field in the detector if 0.5 kV/cm, which corresponds to an electron drift-velocity of 1.5 mm/$\mu$s, as shown in Figure \ref{fig:fdsp-perform_driftfield}.  An electron drifting over the full 3.6 m length of the TPC will require 2.4 ms to travel that distance under those conditions.  If the electron lifetime of the LAr in the TPC is at the 3.0 ms level, then an attenuation of approximately 50$\%$ should be anticipated for these longest drift lengths, as shown in Figure \ref{fig:fdsp-perform_attenuation}.


\begin{dunefigure}[Drift field vs. drift velocity]{fig:fdsp-perform_driftfield}{The ionization drift-velocity in LAr as a function of the electric field present in the LArTPC, for three different values of LAr temperature.  Measured data from the ICARUS experiment is overlaid.}
\includegraphics[width=0.6\textwidth]{DriftField_Vs_Velocity.pdf}
\end{dunefigure}

\begin{dunefigure}[Electron lifetime impact on free electron attenuation]{fig:fdsp-perform_attenuation}{The percentage of free electron attenuation as a function  of the drift length of the electron, shown for several values of electron lifetime.}
\includegraphics[width=0.6\textwidth]{Lifetime_vs_Attenuation.pdf}
\end{dunefigure}

\subsection{Impact of Electronic Noise and Missing Channels}
\label{sec:fdsp-perform-noise}

\begin{dunefigure}[Noise filtering in MicroBooNE LArTPC]{fig:fdsp-perform_noisefilter}{Reproduction of Figure 14 from \textbf{CITE MicroBooNE Noise Paper}, showing raw LArTPC signal (a) before and (b) after offline noise filtering.}
\includegraphics[width=0.85\textwidth]{NoiseFiltering_MicroBooNE.pdf}
\end{dunefigure}


==> far-detector-single-phase/chapter-fdsp-photon-det/pds-bibliography.tex <==
% Collected here for convenience - NOT used in the TeX build. -- NOT complete  4/17/18

% PD Bibiography - not included yet - rjw 2/21/18
%For the TDR, we have created the file common/tdr-citedb.bib to contain all the citations. Please
% read the guidelines at the beginning of that file. We have left a well-populated common/citedb.bib
% in the TDR directory in case you want to search for a citation that may have appeared in the
% CDR, or other DUNE/LBNF document



\begin{thebibliography}{1}
%Denver
\bibitem{bib:JINST-11-C05019}
D.~Whittington.
\newblock Photon detection system designs for the deep underground neutrino
  experiment.
\newblock {\em Journal of Instrumentation}, 11(05):C05019, 2016.

\bibitem{bib:DoubleShiftLG-NIM-171113}
B.~Howard, S.~Mufson, D.~Whittington, B.~Adams, B.~Baugh, J.~Jordan, J.~Karty,
  C.~Macias, and A.~Pla-Dalmau.
\newblock {A Novel Use of Light Guides and Wavelength Shifting Plates for the
  Detection of Scintillation Photons in Large Liquid Argon Detectors}.
\newblock {\em Nucl. Instrum. Meth.} (submitted).
\newblock FERMILAB-PUB-17-488-ND-PPD.
\newblock arXiv:1710.11233.

\end{thebibliography}

\end{document}



\begin{thebibliography}{99}
% Ana
\footnotesize{

\bibitem{arapuca_jinst} A.A. Machado and E. Segreto, Journal of Instrumentation, 11, C02004 (2016).

\bibitem{VIKUITI}
	3M VIKUITY foils. https://en.wikipedia.org/wiki/Vikuiti.
    
\bibitem{arpkLNLS} H. daMotta, A.A. Machado, L. Paulucci, E. Segreto, B. Gelli, M.R. Guzzo, G. Marques, D. Galante, V. Teixeira, W. Araujo, C. Ambrosio, M.Bissiano, F. Marinho. {\bf"ARAPUCA light trap for large liquid argon time projection chambers"}
    https://pos.sissa.it/295/153/pdf

}
\end{thebibliography}

\end{document}


@article{Grace:2015yta,
      author         = "Grace, Emily and Nikkel, James A.",
      title          = "{Index of refraction, Rayleigh scattering length, and
                        Sellmeier coefficients in solid and liquid argon and
                        xenon}",
      journal        = "Nucl. Instrum. Meth.",
      volume         = "A867",
      year           = "2017",
      pages          = "204-208",
      doi            = "10.1016/j.nima.2017.06.031",
      eprint         = "1502.04213",
      archivePrefix  = "arXiv",
      primaryClass   = "physics.ins-det",
      SLACcitation   = "%%CITATION = ARXIV:1502.04213;%%"
}


==> far-detector-single-phase/chapter-fdsp-slow-and-cryo/cryo-instrum-cfd-sp-only.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Cryogenics Instrumentation}

%%% This file is no longer needed -- text added to cryo-instrum-cfd2 July 16 2018 AH to get back to ``Dario's version''
Although simulation of the \dword{detmodule} presents challenges, there exist acceptable simplifications for accurately representing the fluid, the interfacing solid bodies, and variations of contaminant concentrations. Because of the magnitude of thermal variation within the cryostat, modeling of the \dword{lar} is simplified through use of constant thermophysical properties, calculation of buoyant force through use of the Boussinesq Model (using constant a density for the fluid with application of a temperature dependent buoyant force), and a standard shear stress transport turbulence model. Solid bodies that contact the \dword{lar} include the cryostat wall, the cathode planes, the anode planes, the ground plane, and the \dword{fc}. As in previous \dshort{cfd} models of the DUNE \dword{35t} and \dword{protodune} by South Dakota State University (SDSU)\cite{docdb-5915}, the \dword{fc} planes, anode planes, and \dword{gp} can be represented by porous bodies. Since impurity concentration and electron lifetime do not impact the fluid flow, these variables can be simulated as  passive scalars, as is commonly done for smoke releases~\cite{cfd-1} in air or dyes released in liquids.




==> far-detector-single-phase/chapter-fdsp-tpc-elec/fdsp-tpc-elec-design-warm-test.tex <==
The warm interface electronics %must 
provide an interface between the \dword{ce}, \dword{daq}, timing, and slow control systems, including local power control at the flange and a real-time diagnostic readout. They are housed in the \dwords{wiec} attached directly to the \dword{ce} flange.  The \dword{wiec} shown in Figure~\ref{fig:tpcelec-flange} 
contains one power and timing card (\dword{ptc}), five warm interface boards (\dwords{wib}) and a passive
power and timing backplane (PTB), which fans out signals and \dword{lv} power from the \dword{ptc} to the \dwords{wib}. The \dword{wiec} must provide a Faraday-shielded housing, robust ground connections from the \dwords{wib} to the detector ground described in Section~\ref{sec:fdsp-tpc-elec-design-ground}, and only optical fiber links to the \dword{daq} and slow control in order to mitigate noise introduced at the \dword{ce} \fdth.


\begin{dunefigure}
[Exploded view of the \dword{ce} signal flange for \dword{pdsp}.]
{fig:tpcelec-flange}
{Exploded view of the \dword{ce} signal flange for \dword{pdsp}.  The design will be very similar for the \dword{spmod} \dword{ce} signal flange (with two \dword{ce} signal flanges per \fdth).}
\includegraphics[width=0.9\linewidth]{tpcelec-flange.png}
\end{dunefigure}

The \dword{wib} is the interface between the \dword{daq} system and four
\dwords{femb}. It receives the system clock and control signals from the
timing system and provides for processing and fan-out of those signals to the four
\dwords{femb}. The \dword{wib} also receives the high-speed data signals from the four 
\dwords{femb} and transmits them to the \dword{daq} system over optical
fibers. The data signals are recovered onboard the \dword{wib} with commercial equalizers.
The \dwords{wib} are attached directly to the TPC
\dword{ce} \fdth on the signal flange. The \fdth
board is a PCB with connectors to the cold signal and \dword{lv} power cables fitted
between the compression plate on the cold side, and sockets for
the \dword{wib} on the warm side. Cable strain relief for the cold cables is 
supported from the back end of the \fdth.

\begin{dunefigure}
[\dword{pdsp} PTC and timing distribution to the WIB and FEMBs]
{fig:tpcelec-wib_timing}
{Power and timing card (\dword{ptc}) and timing distribution to the \dword{wib} and \dwords{femb} used in \dword{pdsp}.}
\includegraphics[width=0.75\linewidth]{tpcelec-wib_timing.pdf}
\end{dunefigure}

The \dword{pdsp} \dword{ptc} provides a bidirectional fiber interface to the
timing system. The clock and data
streams are separately fanned out to the five \dwords{wib} as shown in
Figure~\ref{fig:tpcelec-wib_timing}. The \dword{ptc} fans the clocks out to the \dword{wib} over the
PTB, which is a passive backplane attached directly to the \dword{ptc} and
\dwords{wib}.  The received clock on the \dword{wib} is separated into clock and
data using a clock-data separator. Timing endpoint firmware to receive and transmit
the clock is integrated in the \dword{wib} \dword{fpga} (the Altera Arria V\footnote{Altera Arria\texttrademark{}, V FPGA family, \url{https://www.altera.com/products/fpga/arria-series/arria-v/overview.html}.} was used for \dword{pdsp}).
The \dword{spmod} timing system, described in Section~\ref{sec:fdsp-daq-timing}, is a development of the \dword{pdsp} system, and expected to require the nearly identical functionality at the \dword{wib} endpoint.

\begin{dunefigure}
[\dword{pdsp} \dword{lv} power distribution to the \dword{wib} and \dwords{femb}]
{fig:tpcelec-wib_power}
{\dword{lv} power distribution to the \dword{wib} and \dwords{femb} implemented for \dword{pdsp}. This will be modified for the \dword{spmod} to provide the required voltage or voltages depending on which \dwords{asic} are used on the \dwords{femb}. In particular the voltages to the \dword{femb} \numrange{0}{3} will change as the \dword{pdsp} \dword{fpga} is replaced by \dword{coldata}. }
\includegraphics[width=0.65\linewidth]{tpcelec-wib_power.pdf}
\end{dunefigure}


The \dword{ptc} also receives \SI{48}{V} \dword{lv} power for all cold
electronics connected through the TPC signal flange: one \dword{ptc}, five \dword{wib}, and \num{20}~\dword{femb}. The \dword{lv} power is then stepped down
to \SI{12}{V} via a DC-DC converter onboard the \dword{ptc}. The output of the \dword{ptc} converters is filtered with a common-mode choke and fanned out
on the PTB to each \dword{wib}, which provides the necessary \SI{12}{V} DC-DC conversions and fans
the \dword{lv} power out to each of the cold \dwords{femb} supplied by that \dword{wib}, 
as shown in Figure~\ref{fig:tpcelec-wib_power}. The output of the \dword{wib} converters are further filtered by a common-mode choke. The 
majority of the power drawn by a full flange is dissipated in the \lar by the cold \dword{femb}.

%Each \dword{wib} contains a 
%unique IP address for its UDP slow control interface. The IP address for the \dword{wib} is 
%derived from a crate and slot address: the crate address is generated on the \dword{ptc} 
%board via dipswitches and the slot address is generated by the PTB slot, numbered 
%from one to five. Note that the \dwords{wib} also have front-panel
%connectors for receiving \dword{lv} power; these can be used in place of 
%the \dword{lv} power inputs on the PTB generated by the \dword{ptc}.

As shown in Figure~\ref{fig:tpcelec-dune_wib}, the \dword{wib} is capable of receiving \dword{lv} power in the front panel and distributing it directly to the \dword{femb}, bypassing all DC/DC converters.
It can also receive the encoded system timing signals over bi-directional optical
fibers on the front panel, and process these using either
the on-board \dword{fpga} or clock synthesizer chip to provide the clock required by the \dword{ce}.
The baseline \dword{asic} design currently uses 8b/10b encoding; if the SLAC CRYO \dword{asic} is selected for
the DUNE \dword{spmod}, 12b/14b encoding will be used instead of 8b/10b.

%\begin{dunefigure}


The \dword{fpga} on the \dword{pdsp} \dword{wib} is an Altera Arria V GT variant, which has
transceivers that can drive the high-speed data to the \dword{daq} system up to
10.3125~Gbps per link, implying that all data from
two \dword{femb} (2$\times$5~Gbps) could be transmitted on a single link.
The \dword{fpga} has an additional Gbps Ethernet transceiver I/O based on the \SI{125}{MHz} clock, which 
provides real-time digital data readout to the slow control system.

